Hierarchical Inducing Point Gaussian Process for Inter-domain Observations

We examine the general problem of inter-domain Gaussian Processes (GPs): problems where the GP realization and the noisy observations of that realization lie on different domains. When the mapping between those domains is linear, such as integration or differentiation, inference is still closed form. However, many of the scaling and approximation techniques that our community has developed do not apply to this setting. In this work, we introduce the hierarchical inducing point GP (HIP-GP), a scalable inter-domain GP inference method that enables us to improve the approximation accuracy by increasing the number of inducing points to the millions. HIP-GP, which relies on inducing points with grid structure and a stationary kernel assumption, is suitable for low-dimensional problems. In developing HIP-GP, we introduce (1) a fast whitening strategy, and (2) a novel preconditioner for conjugate gradients which can be helpful in general GP settings. Our code is available at https: //github.com/cunningham-lab/hipgp.

==> sections/experiments-synthetic.tex <==
% two-dimensional experiment
\subsubsection{Synthetic Two-Dimensional}
\label{sec:experiment-synthetic}
 We synthesize two-dimensional observations function of varying complexity
 from random neural networks with sinusoidal non-linearities,
see the top row of Figure~\ref{fig:synthetic-experiment}.
Below we describe predictive performance as we vary three algorithmic choices:
the number of inducing points $M$, the complexity of the posterior approximate
covariance $\bS$, and the maximum number of PCG iterations allowed for each
solve.

\paragraph{Scaling inducing points}
We compare held out mean absolute eror and
the training time as a function the of number of
inducing points $M$ and the variational approximation complexity.
In this simulation, we fit a model to $N=20{,}000$ observations with
observation noise $\sigma_n = .1$.
%the stochastic gradient descent learning rate to $2^{-2}$ for mean field variational family and $1^{-2}$ for block diagonal variational family, and batch size
%to $100$ and number of epochs to $10$.
For the block-diagonal approximation, we fix the block size $M_b = 100~(10\times10)$.
The results are displayed in Figure~\ref{fig:mae-by-M} and Figure~\ref{fig:time-by-M}.
From this experiment we conclude:
(i) increasing $M$ increases prediction quality;
(ii) the block-diagonal variational covariance outperforms the more
constrained mean field parameterization, and is comparable to full-rank approximation
when the full-rank is feasible; (iii) the HIP-GP is almost indistinguishable to SVGP in predictive performance,
but is faster in large $M$ settings.

%%%%%%%%%%%%%%%%%%%%%%%%%
% Test Functions
%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t!]
  \centering
  \begin{subfigure}{.32\columnwidth}
    \includegraphics[width=\columnwidth]{figures/synthetic/true-fgrid-simple.pdf}
    \caption{simple $\rho(x)$}
		\label{fig:ftrue-simple}
  \end{subfigure}
  \begin{subfigure}{.32\columnwidth}
    \includegraphics[width=\columnwidth]{figures/synthetic/true-fgrid-medium.pdf}
    \caption{medium $\rho(x)$}
  \end{subfigure}
  \begin{subfigure}{.32\columnwidth}
    \includegraphics[width=\columnwidth]{figures/synthetic/true-fgrid-hard.pdf}
    \caption{complex $\rho(x)$}
		\label{fig:ftrue-complex}
  \end{subfigure}
	%\%vspace{.5em}
  \begin{subfigure}{\columnwidth}
		\centering
    \includegraphics[width=.8\columnwidth]{{figures/synthetic/synthetic-mae.pdf}}
    \caption{Predictive error (complex $\rho(x)$).}
    \label{fig:mae-by-M}
  \end{subfigure}
	%\vspace{.5em}
  \begin{subfigure}{\columnwidth}
    \centering
		\includegraphics[width=.8\columnwidth]{{figures/synthetic/synthetic-time.pdf}}
    \caption{Training wallclock time for 10 epochs(complex $\rho(x)$).}
    \label{fig:time-by-M}
  \end{subfigure}
	\caption{HIP-GP performance on synthetic data. Top: two-dimensional synthetic
		test functions.  Middle: predictive mean absolute error (MAE) as a function
		of $M$ and $\bS$ type --- mean field (MF), block diagonal (BD) or full
		rank (which did not scale past $M=3{,}000$).
    %Note that the full-rank lines and the block lines overlap for $M=1{,600}$ to $3{,}600$.
		Bottom: Training wall clock time for 10 epochs.
    HIP-GP takes less time to train for $M \geq10{,}000$.
  }
  \label{fig:synthetic-experiment}
\end{figure}


\paragraph{PCG Iteration Early Stopping}
Additionally, we examine the effect of the maximum number of PCG iterations
when computing $\bk_n = \bK_{\bu,\bu}^{-1}\bK^{}_{\bu,n}$ on approximation
quality.  Figure~\ref{fig:pcg-iter} depicts test
log-likelihood as a function of PCG iteration for a modest-sized $M = 1{,}600$
on the simple test function (in Figure~\ref{fig:ftrue-simple}) for $N=20{,}000$
data.  The full rank solution is computed by a direct solve, however the mean
field and block-diagonal use PCG.  The final approximation
quality is robust to the number of PCG iterations used.  We observe similar
behavior on the medium and complex functions for larger values of $M$.  The
upshot is that the HIP-GP needs only a small number of PCG iterations
to be effective.This early stopping advantage is consistent with conventional
wisdom in the optimization literature.


\begin{figure}[t!]
  \centering
  \includegraphics[width=.7\columnwidth]{figures/synthetic/maxiter-plots/maxitercg-loglike-func=simple.pdf}
  \caption{Stochastic optimization is robust to early stopping PCG iterations.
     %Because of this, we can stop after only 5 to 10 iterations, saving on
     %computation time per iteration.
  }
  \label{fig:pcg-iter}
  %\vspace{-1em}
\end{figure}


==> sections/method-whitened.tex <==
\subsection{Whitened parameterization}
\label{sec:whitened}

Whitened (or non-centered) parameterizations are used to improve
inference in models with correlated priors because they offer a
better-conditioned posterior
\citep{murray2010slice, hensman2015mcmc}.
Here we obtain an additional important computational benefit of it
in the variational setting --- the whitened posterior allows us to
avoid computing $\ln |\bK_{\bu,\bu}|$, a fact that has not been observed
in the literature.
To define the whitened parameterization, we describe the GP prior over
$\bu$ as a deterministic function of standard normal parameters $\bepsilon$
\begin{align}
  \bepsilon \sim \mathcal{N}(0, I) \,, \quad
  \bu = \bK_{\bu,\bu}^{1/2} \bepsilon \sim \mathcal{N}(0, \bK^{}_{\bu,\bu}) \,.
   \label{eq:matrix-sqrt}
\end{align}
We target the posterior over
the \emph{whitened parameters}
$\bepsilon$ with variational approximation
${q_{\blambda}(\bepsilon) = \mathcal{N}(\bepsilon \given \bm, \bS)}$.
The resulting whitened variational objective is
\begin{align*}
\mathcal{L}(\blambda)
  %&= \mathbb{E}_{q_{\blambda}(\epsilon) p(\brho \given \epsilon)}
  %    \left[ \ln p(\by \given \brho) \right] -
  %    KL(q_{\blambda}(\epsilon) \,||\, p(\epsilon)) \\
  &= \sum_{n} \underbrace{
  	    \mathbb{E}_{q_{\blambda}(\bepsilon) p(\brho \given \bepsilon)} \left[
	    	\ln p(y_n \given \rho_n)
	    \right]
	  }_{\circled{$a'_n$}} -
      \underbrace{
	  	KL(q_{\blambda}(\bepsilon) \,||\, p(\bepsilon))
	  }_{\circled{b$'$}} \,
\end{align*}
where
\begin{align}
\circled{$a'_n$}
&= -\frac{1}{2}\ln \sigma_n^2 - \frac{1}{2\sigma_n^2}
    \Big( y_n^2 + \bK^{**}_{n,n} - \bk_n^\intercal \bk^{}_n  \nonumber \\
&\quad + \bk_n^\intercal
     \left( \bS + \bm \bm^\intercal \right) \bk_n - 2 y^{}_n \bk_n^\intercal \bm
    \Big) \,\,,\\
\circled{b$'$}
%KL(q_{\blambda}(\epsilon) \,||\, p(\epsilon))
  &= \frac{1}{2}\left( \text{tr}(\bS) + \bm^\intercal \bm - \ln |\bS| - M \right) \,
\label{eq:kl-term}
\end{align}
 and we define the correlation term for clarity
 \begin{align}
    \bk_n \triangleq Cov(\bepsilon, \be_n)  = \bK_{\bu,\bu}^{-1/2}\bK^*_{\bu,n}  \,\,.
    \label{eq:k-vector}
 \end{align}

Becuase $p(\bepsilon)$ is a standard normal we have simplified term \circled{$b'$},
by avoiding computing $\ln |\bK_{\bu,\bu}|$.
The remaining computational bottlenecks are
the correlation term $\bk_n$ in \circled{$a_n'$} and the $\ln |\bS|$ in \circled{$b'$}
which we address in the following.
Specifically, we note that the efficient computation of $\bk_n$
depends on the specific choice of whitening strategy,
which we will discuss in Section~\ref{sec:computational}.

